Motif-Driven Contrastive Learning of Graph Representations

Pre-training Graph Neural Networks (GNN) via self-supervised contrastive learning has recently drawn lots of attention. However, most existing works focus on node-level contrastive learning, which cannot capture global graph structure. The key challenge to conducting subgraph-level contrastive learning is to sample informative subgraphs that are semantically meaningful. To solve it, we propose to learn graph motifs, which are frequently-occurring subgraph patterns (e.g. functional groups of molecules), for better subgraph sampling. Our framework MotIf-driven Contrastive leaRning Of Graph representations (MICRO-Graph) can: 1) use GNNs to extract motifs from large graph datasets; 2) leverage learned motifs to sample informative subgraphs for contrastive learning of GNN. We formulate motif learning as a differentiable clustering problem, and adopt EM-clustering to group similar and significant subgraphs into several motifs. Guided by these learned motifs, a sampler is trained to generate more informative subgraphs, and these subgraphs are used to train GNNs through graph-to-subgraph contrastive learning. By pre-training on the ogbg-molhiv dataset with MICRO-Graph, the pre-trained GNN achieves 2.04% ROC-AUC average performance enhancement on various downstream benchmark datasets, which is significantly higher than other state-of-the-art self-supervised learning baselines.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle


==> section/_0_method_old.tex <==

\begin{figure*}[h!]
\begin{center}
\includegraphics[width=13.97cm]{picture/framework.png} 
\end{center}
\caption{Overall framework of \textit{\method}. A GNN trained in a self-supervised manner to automatically extract motifs. The learned motifs are leveraged to generate informative subgraphs for graph-to-subgraph contrastive learning.}
\label{figure:framework}
\end{figure*}

\subsection{The Overall Framework of \textit{\method}} \label{subsec:framework}
Graph motif discovery through exact counting is a combinatorial problem, which is hard to generalize to large datasets with continuous or high-dimensional features. We thus propose to formalize motif mining as a differentiable clustering learning problem and solve it by self-supervised representation learning using GNNs. Our goal is to train a GNN encoder that can be used to generate meaningful graph-level representations and extract graph motifs. 

Given a dataset with M graphs $\sG = \{\gG_{1}, ..., \gG_{M} \}$, the differentiable clustering learning problem is meant to learn two things. One is a GNN-based graph encoder $\bm E(\cdot)$ that maps input (sub)graphs to meaningful embedding vectors that captures (sub)graph properties.  The other is a K-slot embedding table $\{\vm_{1}, ..., \vm_{K}\}$, where each slot stores a cluster center of embeddings of frequently occurred subgraph patterns. These K vectors are our motif embedding vectors. Different from the traditional motif that emphasize pattern matching, motif embeddings emphasize more on semantic meanings. This is more useful abstraction, because people study exact patterns for their semantic meanings. It used to be that case that two subgraph patterns differ by a little are considered different motifs, but in our framework they could correspond to the same motif embedding because they share very similar semantic meanings. An example from chemistry would be a sulfate ($-SO_4$) and a phosphate ($-PO_4$), which are considered to be the same motif in our sense and indeed share very similar chemical properties. 


To tackle the differentiable clustering learning problem, we introduce the \textit{\method} framework which consists three modules: 1) a module conducts constrastive learning to train the GNN encoder; 2) a \textit{Motif-Learner} to cluster subgraphs and identify motif embedding vectors. 3) a \textit{Motif-guided Segmenter} to extract informative subgraphs that help the other two modules to train; The overall framework is shown in Figure\ref{figure:framework}. We describe the motivation and design details of these three module in order in the following sections.

\subsection{Challenges and Proposed Solutions of Graph Contrastive Learning} \label{subsec:contrastive}
An expressive GNN encoder $\bm E(\cdot)$ is essential for capturing graph properties and accurately identifying motifs. Since we train the GNN in a self-supervised manner without relying on any labels, we use contrastive learning to guide the training. Contrastive learning is one of the state-of-the-art self-supervised learning methods that achieves great results in vision and language domain (see \ref{sec:related} for a detailed introduction). One key component for the success of contrastive learning is to generate informative and diverse views of data instances. For example, for images, two random crops from the same image can be a pair of positive views, and two random crops from different images can be a pair of negative views. With a pre-defined agreement measure, the encoder is trained to maximize agreement of representations of positive view pairs and minimize agreement of representations of negative view pairs. The intuition, or hidden assumption, of contrastive learning is that a pair of positive views should both capture some common properties of the original data instance, but a negative pair does not since two views come from different instances. For an image of a dog, a positive pair could corresponds to a head crop and a tail crop of the dog, where as a negative pair could corresponds to one crop of the dog and one crop from another image of a cat. 

A direct transformation of this idea from the image domain to the graph domain is to generate two random subgraphs from the same whole graph as a positive pair, and two random subgraphs from different whole graphs as a negative pair, where the sampling may be done by random walk as in many graph learning literature. However, this simple adaption is problematic because most view pairs will be invalid. The reason is intrinsic to the properties of graph data, i.e. the discrete topological structure with coarse granularity, the locality, and the small space, and we now discuss why and how to solve these problems. 

\textbf{Views capturing high-level semantic meanings}. As we mentioned above, contrastive learning only works well when we can generate informative and diverse and views. As an example, for a molecule graph, desired views could mean different subgraphs that capture various chemical properties. The challenge to achieve this is that graphs are discrete topological structures with coarser granularity compared to images. When randomly crop one square piece of an image, pixels in this crop will be highly related. Value of one pixel heavily depends on the other pixels around it. Pixels in this piece will together represent a high-level meaning, which can be an object in the image, like a dog, or maybe just the background, like sky or grass. Also, pixels are fine-grained. When the crop misses some pixels and only captures part of an object, say only half of the dog's head, the high-level meaning is still there. However, for graphs, an edge between two nodes only represents the topological structure. It does not necessarily mean high dependency because of the discreteness. When nodes are two or more hops away, it is much harder to tell the dependency between them. Besides, nodes in graphs are coarser-grained than pixels in images, so even when there is some meaningful substructure like a motif, a sampled subgraph missing one node of the motif structure can mean missing the semantic meaning completely. Under all these conditions, a randomly sampled subgraph is unlikely to have a desired high-level meaning. It is in some sense similar to randomly pick some pixels from an image and use it as a view. 

Therefore, we propose to train a motif-guided segmenter to produce informative subgraphs similar to graph motifs, which helps the GNN to learn higher-level graph information during contrastive learning. Details of motif-guided segmenter will be discussed in \ref{subsec:segmenter}, and comparison between motif-guided segmenter and other heuristic sampling methods are shown in \ref{subsec:ablation}.
Experiment results show that simple heuristic sampling methods lead to bad generalization performance, which demostrates the significance of informative motif-like subgraphs.

% This is because randomly generated subgraphs usually loose the global view, the contextuallized information. It is more likely a collection and aggregation of of node level properties rather than capturing the property of a meaningful micro-structure in the whole graph. Relying on these kind of subgraphs, the model can not learn higher level properties. Thus, the contrastive between them may not make much sense. 

% In order to learn a representation of graphs with global property, we would like the views to contain some higher level information.

% because our goal is to train the GNN to produce meaningful graph-level representations. Ideally, the views we generate should represent some higher-level meanings, Otherwise the contrastive won't be very effective.That is why we need motifs.

\textbf{False positive view pairs}. Even with informative motif-like subgraphs, the contrastive learning still faces the issue of invalid view pairs that break the hidden assumption. For two crops of the same image, even when they have no overlap, there could be many global properties shared by them, e.g. the background, the texture, the hue, and the brightness of the image. In contrast, even sampled from the same whole graph, by locality, two non-overlapped or slightly overlapped subgraphs could be only very weakly related to each other if not non-related. In this case, these two views become a false positive pair, and maximizing their agreement provides wrong learning signals. One may argue that we can increase the overlapping ratio of two views. However, as we would like to generate motif-like subgraphs, high overlapping basically means two views corresponding to the same motif. We thus will lose the diversity of views, which is also undesired, as maximizing the agreement of the already very views is a tautology and doesn't help the model to learn.

% One may argue that we can control the sampling process to make two subgraphs overlap with each other. However, this is a non-trivial task that creates more questions we need to answer. For example, what is the proper overlap ratio? When it is too small, it could be not helpful for the locality issue. When it is too large, the task becomes too easy and the training signal becomes useless, since claiming two subgraphs sharing 90\% nodes are similar is a tautology and doesn't help the model to learn. A high overlap ratio is also contradict to the motif-guided sampling mentioned above. We would like to generate views corresponding to different motifs rather than the same motif. 

To solve the false positive pair problem, we propose graph-to-subgraph contrastive instead of subgraph-to-subgraph contrastive. These two different contrastive strategies correspond to two agreement measures. The subgraph-to-sugraph measure is symmetric, and it measures whether two subgraphs are similar to each other. The graph-to-subgraph measure is asymmetric, and it measures whether the second view captures some aspect of the first view. This design choice considers the global-to-local relationship, which avoids false positives. This global-to-local contrastive is not a new idea, but in previous works, the local views were merely node-level, which is disadvantaged for capturing higher-level information as we discussed above. A possible reason why subgraph views were not used is that knowing how to group nodes to informative subgraphs is challenging, which we solve by the motif-guided training. For the difference of view generation between our model and previous work, please see \ref{figure:contrastive}. Comparison between subgraph-to-subgraph contrastive and graph-to-subgraph contrastive are shown in \ref{subsec:ablation}. Experiment results demonstrate the advantage of the later.

% (For whether the graph-to-subgraph makes sense, please refer to \ref{figure:whole_motif_assign}, that different subgraphs will triger different dimensions of the whole graph.)

\textbf{False negative pairs}. Besides false positive pairs caused by graph locality, there are also false negative pairs caused by small graph space. Compared to the image space, the total dimension of the graph space is much smaller. In general benchmark datasets, there are less nodes in a graph than pixels in an image, and node features also have much smaller dimensions than pixels with three channels.
% usually graph node features are less than ten dimensions and each dimension can only take a few discrete values, where as image pixels have three channels with 256 dimensions each. The means when we sample two subgraphs from different whole graphs, they are likely to be similar to each other. Thus, false negatives. (Move this part to discussion?)
The space is small means when considering a large number of subgraphs sampled from different whole graphs, some of them will likely to have similar structures and contain similar nodes. 
Consider subgraphs $g1$ and $g2$ sampled from whole graphs $\gG_1$ and $\gG_2$ respectively. When $g1$ and $g2$ are very similar to each other, the pair ($\gG_1$, $g2$) is problematic, because $g_2$ is working effectively as $g_1$, but we label the pair negative. This is what we call the false negative pair problem.

To tackle this issue, we propose to use contextualized embedding to do contrastive learning. What motivated this idea is again the image example. Image crops from different big images are unlikely to be very similar. One way to think about it is the large space, so statistically it is unlikely. Another way to think about it is that global information is be used to distinguish different crops, like the background, texture, hue, and brightness as we discussed above. Even for two images of the same object, it is very unlikely for them to have consistent global information in all perspectives. By contextualized embedding we are actually referring to embeddings with global information, e.g. a subgraph embedding with messages collected from a much larger region and more nodes than only nodes within it. Specifically, when generating the subgraph embeddings, we first generate all the node embeddings by doing GNN message passing on the entire whole graph. After this step, all the nodes will contain information of a large graph region, and thus contextualized. Here the region size depends on the number of GNN layers. Then we use motif-guided segmenter to decide which nodes we want to put together as a subgraph and group them accordingly. The subgraph embedding will be an aggregation of these contextualized node embeddings, which will not only contain the local information from nodes within this subgraph, but also contextual information about the whole graphs. Using the example we give above, even
though $g_1$ and $g_2$ can be similar, their embeddings $\vs_1$ and $\vs_2$, which we actually use for contrastive loss computation, are different. Comparison between regular subgraph embeddings and contextualized subgraph embeddings are shown in \ref{subsec:ablation}. Experiments show the advantage of the later.

\textbf{Contrastive learning summary}. For the most effective contrastive learning on graphs, we propose three different solutions to overcome the corresponding difficulties. We use motif-guided segmenter to generate more informative subgraphs as one of our views, and use whole graph as the other view for a global-to-local contrastive to avoid false positive pairs, and also contextualized embeddings to avoid false negative pairs.

To put everything more concretely. Given a dataset with M graphs $\sG = \{\gG_{1}, ..., \gG_{M} \}$, $J_i$ subgraphs will be generated by the motif-guided segmenter from $\gG_{i}$. In total, there will be $J = \sum_{i=1}^{M} J_i$ subgraphs. We denote the embedding of these whole graphs and subgraphs as $\{\vh_1, ..., \vh_M\}$ and $\{\vs_1, ..., \vs_J\}$ respectively. Then we compute the graph-to-subgraph similarity matrix $\mW \in \R^{M \times J}$, where the entry $(i, j)$ is the cosine similarity between the corresponding graph-subgraph pair, i.e. $\emW_{i, j} = \phi(\vh_{i})^T \phi(\vs_{j})$\footnote{For notation simplicity, we denote a L-2 normalization operator by $\phi(\cdot)$ such that $\phi(x) = x \ / \ \Vert x \Vert_{2}$.}. For the whole graph $\gG_i$, subgraphs sampled from it are considered as positive pairs to it, and subgraphs sampled from other graphs are considered as negative pairs to it. Then the contrastive objective function is the following, where we do row-wise softmax normalization with temperature parameter $\tau_g$ :
\begin{equation}
    {\cal L}_c  = -\frac{1}{M} \sum_{i=1}^{M} \sum_{j = 1}^{J}  \1\{g_j \in \gG_i\} \cdot \log \frac{\exp(\emW_{i, j} / \tau_g)}{\sum_{j'}\exp(\emW_{i, j'} / \tau_g)} 
\end{equation}

\begin{figure*}[h]
\begin{center}
\includegraphics[width=13.97cm]{picture/contrastive.png} 
\end{center}
\caption{ Different ways to generate views for graph data. Context Prediction uses one node and one context graph as views. InfoGraph uses one node and the whole graph as views. Our method uses a higher-level subgraph as one view and the whole graph as another; thus the GNN can capture more global contextual information. }
\label{figure:contrastive}
\end{figure*}
% aims to simutaneously learn subgraph representations and cluster these representations based on their semantic meaning. The first step is to do clustering on data representations and get a (soft) cluster assignment for each representation. The second step is to use cluster assignments learned in the first step as labels to update representations.

\subsection{Motif Learner via EM Clustering}\label{subsec:motif_learner}
In this section, we describe how do we learn the motif embeddings with the \textit{Motif Learner}. The main idea is to model and optimize the similarity between subgraphs and motifs through an Expectation-Maximization (EM) style clustering algorithm on sampled subgraphs. We start with K randomly initialized motif embeddings vectors $\{\vm_{1}, ..., \vm_{K}\}$ and $J$ subgraph embeddings $\{\vs_1, ..., \vs_J\}$ generated from the motif-guided segmenter.

\textbf{E-Step.} During the E-step, we assume all the embeddings are fixed, and our goal is to come up with an optimal assignment matrix that cluster each subgraph embedding to one of the $K$ motif clusters. We denote the assignment matrix by $\mQ \in \R^{K \times J} $, where the $j$-th column contains the probabilities of assigning the $j$-th subgraph to each of the K motifs, so that $\emQ_{k,j} \in [0, 1]$ and $\sum_{k} \emQ_{k,j} = 1$. To find an optimal $\mQ$, we first calculate the pairwise cosine similarity between all the motif embeddings and subgraph embeddings, which we denote using a matrix $\mZ \in \R^{K \times J}$, where the entry (k, j) is $\emZ_{k, j} = \phi(\vm_{k})^T\phi(\vs_{j})$. The optimal assignment we desire, $\mQ^*$, is the one that maximizes similarities between subgraph embeddings and its assigned motif embeddings, i.e. $\mQ^* = \argmax_{\mQ} Tr(\mQ^T \mZ)$.

This objective works fine for a traditional EM clustering algorithm when embeddings are fixed. However, when we do the joint training all modules, the embeddings will constantly change as we are learning and updating model parameters. This vanilla objective will thus lead to a degenerate solution, i.e. all embeddings collapse to a single cluster center. To avoid this issue, we adopt the strategy used in \cite{asano2020self} to solve for $\mQ$ under a slightly modified problem. The modifications include an entropy term $H(\bm{Q}) = - \sum_{i,j}\emQ_{i,j} \log \emQ_{i,j}$ added to the objective and a constraint to restrict the searching space of $\mQ$:
% the constraint set $\cal Q$ requires the marginal projection of $\bm Q$ onto its columns and rows to be uniform.
\begin{equation}
    {\cal Q} = \{ \bm{Q} \in \mathbb{R}_+^{K, J} | \bm{Q 1_{J}} = \frac{\bm{1_K}}{K}, \bm{Q 1_{K}} = \frac{\bm{1_J}}{J} \} 
\end{equation}
where $\bm{1_{N}}$ and $\bm{1_{K}}$ are all one vectors. 

Therefore, the final objective thus becomes the following with lambda being a hyper-parameter. In practice, it will be set to some relatively large number to reduce the influence of $H(\bm{Q})$.
\begin{equation}
    \max_{\bm Q \in \cal{Q}} Tr(\bm{Q}^T \mZ) + \frac{1}{\lambda} H(\bm{Q})
\end{equation}
For more reasons about why this new objective can help avoid the degenerate solution and why it gives a reasonable approximation of $\mQ^*$, we refer the readers to \cite{asano2020self}. Here we will only mention one good property that motivates us to choose this modified optimization problem, which is this problem has a closed-form solution showing in (\ref{eq: sinkhorn}).
\begin{equation} \label{eq: sinkhorn}
    \mQ  = diag(\vu) \cdot \exp(\lambda \mZ) \cdot diag(\vv)
\end{equation}
Here $\bm u$ and $\bm v$ are merely normalization vectors, which can be solved efficiently using a fast Sinkhorn-Knopp algorithm as shown in \cite{cuturi2013sinkhorn}.

\textbf{M-Step.} The goal of the M-step is to maximize the log-likelihood of our data given the cluster assignment matrix $\mQ$ estimated in the E-step. We update parameters in the GNN encoder and the motif embedding table through the M-step. This step is equivalent to a supervised K-class classification problem with labels $\mQ$ and prediction scores $\mZ$. Thus, we first apply a columnwise softmax normalization with temperature $\tau_s$ to $\mZ$ to convert all entries of $\mZ$ to probabilities. Then we use the negative log-likelihood as the loss function.
    
% Specifically, we predict the probability of a subgraph embedding belonging to each cluster, and we optimize the cross entropy loss using values in $\bm Q$ as labels. 
\begin{equation} 
    {\cal L}_m  = -\frac{1}{J} \sum_{j=1}^{J} \sum_{k = 1}^{K} \emQ_{k, j} \log \frac{\exp(\emZ_{k, j} / \tau_s)}{\sum_{j'}\exp(\emZ_{k, j'} / \tau_s)}
\end{equation}


\subsection{Motif-guided Subgraph Segmenter}\label{subsec:segmenter}
When we discuss the contrastive learning and motif learner in the previous two sections, we assumed we have motif-like informative subgraphs. In this section, we describe how can we actually generate these subgraphs.

Sampling subgraphs is a very common operation in graph learning. Some simple approaches showing up often in literature include random walk and k-hop neighbours. The problem of these two sampling methods is that they are only heuristic and cannot accurately capture meaningful subgraphs. Another common approach is node clustering, for example, spectral clustering. A node clustering algorithm segments the whole graph into multiple pieces, and each piece can be treated as a subgraph. The problem of spectral clustering is that there is less randomness as it is not really doing sampling. With a fixed number of clusters, the subgraphs will stay unchanged. More importantly, for all of these approaches, the sampling step considers only the graph structure but not graph features. Thus, it is hard to accurately generate semantically meaningful subgraphs when graph features are critical for representing the (sub)graph properties. We propose to leverage the learned graph motifs to design the \textit{Motif-guided segmenter}, which will learn to segment a given graph into several subgraphs that are close to some discovered motifs. Also, the learning step will consider both graph structure graph feature information.

% it requires expensive eigen-decomposition of the graph adjacency matrix, which can be slow for large graphs. Also,

% For example, heuristically sampled molecule subgraphs are likely to be a chain of carbons, which doesn't contain much information about the original molecule, or it can be a fragment of a meaningful chemical structure, which loses the original chemical property.

\textbf{Subgraph Sampling via Node Clustering.}
The motif-guided segmenter generates motif-like sugraphs by modeling how likely a node will show up in each motif. Given a graph $\gG_i$ with nodes $\{n_1, ..., n_{N_i}\}$, we define an assignment matrix $\mC^{(i)} \in \R^{N_i \times K}$, such that its entry $(j, k)$ represents the probability of node $j$ being part of motif $k$, i.e. $\emC_{j,k}^{(i)} = P(n_j \in \vm_k |\gG_i )$. Here we slightly abuse notation to use $\vm_k$ to represent a motif instantiation of the abstract motif embedding vector. 

To generate subgraphs from $\mC^{(i)}$, we first get the discretized assignment matrix $\tilde \mC^{(i)}$, where there is only one determined motif assignment per each node, i.e. $\tilde \emC_{j, k}^{(i)} = \1\{ \emC_{j, k}^{(i)} = \max_{k} \emC_{j, k}^{(i)}\}$. Our subgraph samples are the induced subgraphs of nodes belong to the same motif. This sampling method guarantees each generated subgraph will likely to be similar to a particular motif, since all the nodes in it have high probability being part of that motif. One note is that we set a threshold $\eta$ indicates the minimum subgraph size we want to have. During sampling, only induced subgraphs with size larger than $\eta$ are generated. In other words, we only produce a subgraph similar to $\vm_j$ if $\sum_i \tilde \emC_{i, j} >= \eta$. This helps us to filter small fragments in a graph that is not considered to be part of any motifs.

Now the problem becomes how should we model this assignment matrix $\mC{(i)}$. We would like to include both the structural information and the features information in our model. Node embeddings from the GNN encoder $\bm E(\cdot)$ provides enough feature information of each node. We can apply a similar clustering procedure on the node level embeddings as we did for subgraphs in \ref{subsec:motif_learner}, so we generate node embeddings $\{\ve_1, ..., \ve_{N_i} \}$ of all $N_i$ nodes in $\gG_i$. Then we compute the cosine similarity between node and motif embeddings as $\emS_{j, k}^{(i)} = \phi(\ve_{j})^T\phi(\vm_{k})$. A further softmax normalization with temperature $\tau_n$ gives the result, $\mC_{j, k}^{(i)} = \frac{\exp(\emS_{j, k} / \tau_n)}{\sum_{k'}\exp(\emS_{j, k'} / \tau_n)}$. 

After that we connect all $M$ assignment matrix to get the total $N = \sum_i N_i$ assignment, i.e. $\mS = \mid\mid \mS^{(i)}$. Then we follow the clustering loss in \ref{subsec:motif_learner} to use the Sinkhorn-Knopp algorithm to produce an optimal assignment $\mP$, as how we calculated $\mQ$ in equation \ref{eq: sinkhorn}. The loss function is thus the negative log likelihood as above.

\begin{equation} 
    {\cal L}_{n}  = -\frac{1}{N} \sum_{i=1}^{M}\sum_{j=1}^{N_i} \sum_{k = 1}^{K} \emP_{j, k} \log \emC_{j, k}^{(i)}
\end{equation}

The shortcoming of this approach is that the graph structure information is only used implicitly during the GNN message passing. This could result in an assignment rely too much on the feature information and assign node with the same feature to the same motif without looking at the structural difference. To capture the structural information more explicitly, we consider penalizing the difference between our clustering result and the result of spectral clustering. As spectral clustering performs really well in finding connected regions within a graph, the penalized loss will balance the feature and structural information. 

We show a regularization term proposed by Bianchi et al. in equation \ref{eq: mincut} \yrcite{bianchi2020spectral}. This regularization is a differentiable approximation of the spectral clustering. As Bianchi et al. mentioned in their paper, this regularizer term should be trained together with other task specific loss to find the optimal trade-off between task-specific and spectral clustering objectives, which is a perfect fit for our purpose. We refer readers to the paper for more discussion about how this loss server the role.

\begin{sequation}  \label{eq: mincut}
    {\cal L}_{r} \! = \!\frac{1}{M} \!\sum_{i = 1}^{M} \!-\frac{Tr(\mC^{(i) T}\!\mA^{(i)}\! \mC^{(i)})}{Tr(\mC^{(i)T}\!\mD^{(i)}\!\mC^{(i)})} + \bigg\Vert\frac{\hat\mC^{(i)T}\!\hat\mC^{(i)}}{\Vert\hat\mC^{(i)T}\!\hat\mC^{(i)}\Vert_{F}} - \frac{\mI_{J_i}}{\sqrt{J_i}}\bigg\Vert_{F}
\end{sequation}

% \begin{sequation}  \label{eq: mincut}
%     {\cal L}_{r} \! = \!\frac{1}{M} \!\sum_{i = 1}^{M} \!-\frac{Tr(\hat\mC^{(i) T}\!\mA^{(i)}\! \hat\mC^{(i)})}{Tr(\hat\mC^{(i)T}\!\mD^{(i)}\!\hat\mC^{(i)})} + \bigg\Vert\frac{\hat\mC^{(i)T}\!\hat\mC^{(i)}}{\Vert\hat\mC^{(i)T}\!\hat\mC^{(i)}\Vert_{F}} - \frac{\mI_{J_i}}{\sqrt{J_i}}\bigg\Vert_{F}
% \end{sequation}

% too long
% \begin{equation}  \label{eq: mincut}
%     {\cal L}_{spec}  = \frac{1}{M} \sum_{i = 1}^{M} -\frac{Tr(\hat\mC^{(i) T}\mA^{(i)} \hat\mC^{(i)})}{Tr(\hat\mC^{(i)T}\mD^{(i)}\hat\mC^{(i)})} + \bigg\Vert\frac{\hat\mC^{(i)T}\hat\mC^{(i)}}{\Vert\hat\mC^{(i)T}\hat\mC^{(i)}\Vert_{F}} - \frac{\mI_{J_i}}{\sqrt{J_i}}\bigg\Vert_{F}
% \end{equation}

where $||\cdot||_{F}$ denotes the Frobenius norm, $\mA^{(i)}$ is the adjacency matrix with self-loop, $\mD^{(i)}$ is the degree matrix of $\mA^{(i)}$, and $\hat\mC^{(i)}$ is the assignment matrix with only $J_i$ selected columns, i.e. only the motifs we are producing corresponding subgraphs.

Putting two terms together, the final loss for training the sampler is
\begin{equation}
    {\cal L}_s =  {\cal L}_{n} + {\cal L}_{r}
\end{equation}

% As this is just an regularization term, we won't let the regularization term dominate and the result matches exactly with the spectral clustering result.
% However, the spectral clustering requires eigen-decomposation, which is hard and slow. Therefore, we use the min-cut loss proposed in minCut pooling to approximate the spectral clustering. For more details about how to use this objective to approximate spectral clustering . Please refer to \cite{bianchi2020spectral}. 


% Our sampling strategy has two advantages over simple sampling strategies like random walk and k-hop neighbors. First, it generates samples utilizing both graph structure and feature information. This is because the sampling result depends on node representations, and the node representations contain both structure and feature information through the message passings in GNN. If the similarity score of a subgraph to the kth motif is higher than some threshold $\eta_k$, we use the following loss term to encourage nodes within this subgraph to become even similar to each other. 


% An example of subgraphs produced by our sampler after training can be found in Appendix \ref{appendix:sampler}


\subsection{Joint training}
The whole framework of \textit{\method} is end-to-end and can be trained jointly with a weighted sum of all three loss terms described above.
\begin{equation}
{\cal L} =  \lambda_m {\cal L}_m + \lambda_s {\cal L}_s + \lambda_c {\cal L}_c
\end{equation}

This objective allow us to simultaneously train an expressive GNN encoder and learn motifs of the given graph dataset. When the training starts, the motif embeddings are randomly initialized and the motif-like subgraphs are rather random. As the training goes, the motif-learner and the motif-guided segmenter will mutually enhance each other and produce better motifs and motif-like subgraphs. We visualize the these results in Figure \ref{figure:motif}

\begin{figure}[ht]
\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{picture/top_motifs.png}}
\caption{Top-6 frequently occurred motifs, represented by their closest subgraph.}
\label{figure:motif}
\end{center}
\vskip -0.2in
\end{figure}


% Pseudocode of our approach is shown in Algorithm \ref{algo:main}. First, we initialize the motif vectors and GNN encoder (line 2 - 3). For each batch of graphs $\sG = \{\gG_{i}\}_{i=1}^{B}$, the segmenter calculates the node-node affinity matrices $\mA^{(i)}$s and extract subgraphs based on the affinity scores (line 5 - 6). After that, GNN message passing is applied on whole graphs to get node embeddings, which are aggregate for both graph and subgraph embeddings (line 7 - 9). The next step is to compute the motif-to-subgraph similarity matrix $\mZ$. Using $\mZ$ we compute both the threshold $\eta$ and cluster assignment matrix $\mQ$ (line 11 - 13). With all these values, the three loss terms and the final joint loss introduced above can be computed (line 15 - 20).

% \begin{algorithm}[H]
% \lstset{style=style_full}
% \begin{lstlisting}[language=Python]
% # temperature parameters: tau_g, tau_n, weight parameters: lamb_m, lamb_c, lamb_s
% model = Motif(args) # model contains all motif vectors, model.motifs
% encoder = GNN(args) # GNN encoder for pre-training
% for G in loader:
%     #I: node index of subgraph,  A: affinity matrices, num_subs: # of subgraphs per graph
%     I, num_subs, A = segmenter(G, encoder) 
%     n = encoder(G)
%     h = aggregate(n, G) # M x D
%     e = aggregate(n, G, I) # N x D
%     S = pairwise_cosine_sim(model.motifs, e) # K x N
%     with torch.no_grad(): 
%         eta = topk_threshold(S) # take the topk similarity scores
%         Q = sinkhorn(S) # use the Sinkhorn-Knopp to solve for Q
        
%     loss_s = sampler_loss(A, eta)
%     S_tilde = torch.softmax(S / tau_g, dim=0) # K x N
%     loss_m = motif_loss(Q, S_tilde)
%     W = torch.softmax(pairwise_cosine_sim(h, e)/tau_g, dim=1)
% 	loss_c = contrastive_loss(W, num_subs) # need num_subs from segmenter   
%     loss = lamb_m*loss_m + lamb_c*loss_c + lamb_s*loss_s
% \end{lstlisting}

% \caption{Pseudocode of MICRO-Graph in PyTorch Style, full version in Appendix \ref{appendix:code}}
% \label{algo:main}
% \end{algorithm}


% (For whether the graph-to-subgraph makes sense, please refer to \ref{figure:whole_motif_assign}, that different subgraphs will triger different dimensions of the whole graph.)

% Moreover, the motif learning and contrastive learning are mutually reinforced: a better GNN produces more accurate subgraph embeddings and thus help motif mining, while better motifs can help generate more informative graph-to-subgraph views and benefit contrastive learning.



==> section/_0_method_old2.tex <==

\begin{figure*}[h!]
\begin{center}
\includegraphics[width=\textwidth]{picture/framework.png} 
\end{center}
\caption{Overall framework of \textit{\method}. A GNN trained in a self-supervised manner to automatically extract motifs. The learned motifs are leveraged to generate informative subgraphs for graph-to-subgraph contrastive learning.}
\label{figure:framework}
\end{figure*}

\subsection{The Overall Framework of \textit{\method}} \label{subsec:framework}
Graph motif discovery through exact counting is a combinatorial problem, which is hard to generalize to large datasets with continuous or high-dimensional features. We thus propose to formalize motif mining as a differentiable clustering learning problem using GNNs.

% Our goal is to train a GNN encoder via contrastive learning to generate meaningful (sub)graph level representations, based on which to extract graph motifs. The learned motifs can reversely benefit the contrastive learning.

Given a dataset with M graphs $\sG = \{\gG_{1}, ..., \gG_{M} \}$, 
% the differentiable clustering learning problem
our goal is to learn two things. One is a GNN-based graph encoder $\bm E(\cdot)$ that maps input (sub)graphs to meaningful embedding vectors that captures their semantic properties.  The other is a $K$-slot motif embedding table $\{\vm_{1}, ..., \vm_{K}\}$, where each slot stores a cluster center of embeddings of frequently occurred subgraph patterns. These $K$ vectors are our motif embedding vectors. 




% This is more useful abstraction because people study exact patterns for their semantic meanings. 
% It used to be that case that two subgraph patterns differ by a little are considered different motifs, but in our framework they could correspond to the same motif embedding because they share very similar semantic meanings. 

% This is especially useful because some structurally similar graphs can deliver very different properties.


% An example from chemistry would be a sulfate ($-SO_4$) and a phosphate ($-PO_4$). Although these two functional groups don't match exactly, they are considered to be the same motif in our sense and they indeed share very similar chemical properties. 


To tackle the differentiable clustering learning problem, we propose the \textit{\method} framework which consists two modules for solving the two research questions we mentioned above.
\begin{compactitem}
    \item A \textit{Motif-Learner} to sample motif-like subgraphs and extract graph motifs by clustering these subgraphs.
    \item A contrastive learning module leveraging graph motifs for self-supervised GNN-based representation learning.
\end{compactitem}

The overall framework is shown in Figure\ref{figure:framework}. We describe the details of these two modules in order in the following sections.

\subsection{Motif Learner: Motif-like Subgraph Sampling and EM Clustering}\label{subsec:motif_learner}
In this section, we describe how do we learn the motif embeddings with the \textit{Motif Learner}. The main idea is to first generate motif-like subgraphs and then optimize the similarity between these subgraphs and the motifs through an Expectation-Maximization (EM) style clustering algorithm. 

In the \textit{Motif Learner}, we model the input data at two different levels, i.e. the relationship between nodes and motifs, and the relationship between subgraphs and motifs. For each $\gG_{i}$ in $\sG$, we denote its $N_i$ nodes by $\{n_{1}^{(i)}, ..., n_{N_i}^{(i)} \}$ and $J_i$ subgraphs sampled from it by $\{g_{1}^{(i)}, ..., g_{J_i}^{(i)} \}$. We use K-way categorical random variables $C_l^{(i)}$ to denote which motif a node belongs to.
\begin{equation}
    P(C_l^{(i)} = k) = P(n_{l}^{(i)} \in \vm_k), \text{ for } 1 \leq k \leq K
\end{equation}
Similarly, we use K-way categorical random variables $Z_j^{(i)}$ to denote which motif a subgraph is similar to.
\begin{equation}
    P(Z_j^{(i)} = k) = P(g_{j}^{(i)} \sim \vm_k), \text{ for } 1 \leq k \leq K
\end{equation}

Here we slightly abuse notation to use $\in$ and $\sim$ to denote the ``belongs to" and ``similar to" relationship.

% We start with K randomly initialized motif embeddings vectors $\{\vm_{1}, ..., \vm_{K}\}$ and $J$ subgraph embeddings $\{\vs_1, ..., \vs_J\}$ generated from the motif-guided Sampler. 

\textbf{Motif-like subgraph sampling}. We sample motif-like subgraphs from a graph $\gG_i$ through the motif assignment of each node in $\gG_i$. We denote the assignments as $Q^{(i)} \in \{0,1\}^{N_i \times K} $. Here the $l$th row $Q^{(i)}_l$ is an one-hot vector represents which motif $n_l^{(i)}$ is assigned to, i.e. $\sum_{k} Q^{(i)}_{l,k} = 1, \forall 1 \leq l \leq N_i$. Then we consider the induced subgraphs of nodes belonging to the same motif as our samples. In other words, for each column $k$ of $Q^{(i)}$, if $\{n_l \vert Q^{(i)}_{l, k} = 1\} \neq \emptyset$, we generate an induced subgraph with these nodes.\footnote{In practice, instead of considering all nonempty node sets, we can set a threshold $\eta$ and only consider $|\{n_l \vert Q^{(i)}_{l, k} = 1\} | > \eta$ to filter out small subgraphs.} When sampling from $M$ input graphs, we denote the assignments of all $N = \sum_{i=1}^M N_i$ nodes as $\mQ = [Q^{(1)}, ..., Q^{(M)}]$. 

The optimal assignment $\mQ^*$ is the one that maximizes the joint probability of all $C_{l}^{(i)}$'s, i.e. the random vector $\mC = [C_1^{(1)}, ..., C_{N_1}^{(1)}, C_{1}^{(2)}, ..., C_{N_M}^{(M)}]$. This $\mQ^*$ guarantees each generated subgraph will likely to be similar to a particular motif, since all the nodes in it have high probability being part of that motif. Formally, this can be written as a constrained optimization problem.
\begin{gather}
\mQ^* = \argmax_{\mQ} Tr(\mQ^T \mC)\\
\text{s.t. } \mQ \in \{0, 1\}^{N \times K} \text{ and } \sum_{k} \mQ_{l,k} = 1, \forall 1 \leq l \leq N \nonumber
\end{gather}
We need to model $\mC$ to solve for $\mQ^*$. Thus, we first get $N_i$ node embeddings in $G_i$, i.e. $\{\ve_{l}^{(i)}\}_{l=1}^{N_i} = \bm E (G_i)$, and then we model $C^{(i)}$ as pairwise cosine similarities between node embeddings and motif embeddings, followed by a softmax normalization to turn values probabilities.
\begin{equation}
C^{(i)}_{l, k} = \frac{\exp(\phi(W_n \ve_{l}^{(i)})^T\phi(\vm_{k}) / \tau_n)}{\sum_{l'}\exp(\phi(W_n \ve_{l'}^{(i)})^T\phi(\vm_{k}) / \tau_n)}
\end{equation}
Here we use $\phi(x) = x \ / \ \Vert x \Vert_{2}$ to denote the L-2 normalization, and $\tau_n$ is a temperature parameter. Also, we project $\ve_{l}^{(i)}$ with a projection parameter matrix $W_n$ in order to capture the asymmetric ``belongs to" relationship.


We first calculate the pairwise cosine similarity between all the motif embeddings and subgraph embeddings, which we denote using a matrix $\mZ \in \R^{K \times J}$, where the entry (k, j) is $\emZ_{k, j} = \phi(\vm_{k})^T\phi(\vs_{j})$. 



This objective works fine for a traditional EM clustering algorithm when embeddings are fixed. However, when we do the joint training all modules, the embeddings will constantly change as we are learning and updating model parameters. This vanilla objective will thus lead to a degenerate solution, i.e. all embeddings collapse to a single cluster center. To avoid this issue, we adopt the strategy used in \cite{asano2020self} to solve for $\mQ$ under a slightly modified problem. The modifications include an entropy term $H(\bm{Q}) = - \sum_{i,j}\emQ_{i,j} \log \emQ_{i,j}$ added to the objective and a constraint to restrict the searching space of $\mQ$:
% the constraint set $\cal Q$ requires the marginal projection of $\bm Q$ onto its columns and rows to be uniform.
\begin{equation}
    {\cal Q} = \{ \bm{Q} \in \mathbb{R}_+^{K, J} | \bm{Q 1_{J}} = \frac{\bm{1_K}}{K}, \bm{Q 1_{K}} = \frac{\bm{1_J}}{J} \} 
\end{equation}
where $\bm{1_{N}}$ and $\bm{1_{K}}$ are all one vectors. 

Therefore, the final objective thus becomes the following with lambda being a hyper-parameter. In practice, it will be set to some relatively large number to reduce the influence of $H(\bm{Q})$.
\begin{equation}
    \max_{\bm Q \in \cal{Q}} Tr(\bm{Q}^T \mZ) + \frac{1}{\lambda} H(\bm{Q})
\end{equation}
For more reasons about why this new objective can help avoid the degenerate solution and why it gives a reasonable approximation of $\mQ^*$, we refer the readers to \cite{asano2020self}. Here we will only mention one good property that motivates us to choose this modified optimization problem, which is this problem has a closed-form solution showing in (\ref{eq: sinkhorn}).
\begin{equation} \label{eq: sinkhorn}
    \mQ  = diag(\vu) \cdot \exp(\lambda \mZ) \cdot diag(\vv)
\end{equation}
Here $\bm u$ and $\bm v$ are merely normalization vectors, which can be solved efficiently using a fast Sinkhorn-Knopp algorithm as shown in \cite{cuturi2013sinkhorn}.

\textbf{E-Step.} During the E-step, we will first sample $J_i$ motif-like subgraphs $\{g_{1}^{(i)}, ..., g_{J_i}^{(i)} \}$ from each $\gG_i$ and then figure out an optimal $Z_j^{(i)}$ value for each of these subgraphs.



\textbf{M-Step.} The goal of the M-step is to maximize the log-likelihood of our data given the cluster assignment matrix $\mQ$ estimated in the E-step. We update parameters in the GNN encoder and the motif embedding table through the M-step. This step is equivalent to a supervised K-class classification problem with labels $\mQ$ and prediction scores $\mZ$. Thus, we first apply a columnwise softmax normalization with temperature $\tau_m$ to $\mZ$ to convert all entries of $\mZ$ to probabilities. Then we use the negative log-likelihood as the loss function.
    
% Specifically, we predict the probability of a subgraph embedding belonging to each cluster, and we optimize the cross entropy loss using values in $\bm Q$ as labels. 
\begin{equation} 
    {\cal L}_m  = -\frac{1}{J} \sum_{j=1}^{J} \sum_{k = 1}^{K} \emQ_{k, j} \log \frac{\exp(\emZ_{k, j} / \tau_m)}{\sum_{j'}\exp(\emZ_{k, j'} / \tau_m)}
\end{equation}

Different from the traditional motif that only considers structural patterns, the motif embeddings in our framework can group structurally-dissimilar subgraphs that share similar semantic meanings into a motif slot.
% This is more useful abstraction because people study exact patterns for their semantic meanings. 
% It used to be that case that two subgraph patterns differ by a little are considered different motifs, but in our framework they could correspond to the same motif embedding because they share very similar semantic meanings. 
% This is especially useful because some structurally similar graphs can deliver very different properties.
An example from chemistry would be a sulfate ($-SO_4$) and a phosphate ($-PO_4$). Although these two functional groups don't match exactly, they are considered to be the same motif in our sense and they indeed share very similar chemical properties. 


\subsection{Motif-guided Subgraph Sampler}\label{subsec:Sampler}
The \textit{Motif Learner} extracts motif embeddings by clustering subgraph embeddings, so that generating informative motif-like subgraph samples is a crucial step for the motif learning. We thus propose to leverage the learned graph motifs to design the \textit{Motif-guided Sampler}, which is superior to simple graph sampling methods often used in previous works (see section \ref{ablation:sample} for more discussion). The \textit{Motif-guided Sampler} learns to segment a given graph into several subgraphs that are close to some discovered motifs. Also, the learning step will consider both graph structure and graph feature information.

% it requires expensive eigen-decomposition of the graph adjacency matrix, which can be slow for large graphs. Also,

% For example, heuristically sampled molecule subgraphs are likely to be a chain of carbons, which doesn't contain much information about the original molecule, or it can be a fragment of a meaningful chemical structure, which loses the original chemical property.

\textbf{Subgraph Sampling via Node Clustering.}
The motif-guided Sampler generates motif-like sugraphs by modeling how likely a node will show up in each motif. Given a graph $\gG_i$ with nodes $\{n_1, ..., n_{N_i}\}$, we define an assignment matrix $\mC^{(i)} \in \R^{N_i \times K}$, such that its entry $(j, k)$ represents the probability of node $j$ being part of motif $k$, i.e. $\emC_{j,k}^{(i)} = P(n_j \in \vm_k |\gG_i )$. Here we slightly abuse notation to use $\vm_k$ to represent a motif instantiation of the abstract motif embedding vector. 

Once we have $\mC^{(i)}$, we can based on it to generate subgraphs. We first get the discretized assignment matrix $\tilde \mC^{(i)}$, where there is only one determined motif assignment per each node, i.e. $\tilde \emC_{j, k}^{(i)} = \1\{ \emC_{j, k}^{(i)} = \max_{k} \emC_{j, k}^{(i)}\}$. Our subgraph samples are the induced subgraphs of nodes belong to the same motif. This sampling method guarantees each generated subgraph will likely to be similar to a particular motif, since all the nodes in it have high probability being part of that motif. One note is that we set a threshold $\eta$ indicates the minimum subgraph size we want to have. During sampling, only induced subgraphs with size larger than $\eta$ are generated. In other words, we only produce a subgraph similar to $\vm_j$ if $\sum_i \tilde \emC_{i, j} >= \eta$. This helps us to filter small fragments in a graph that is not considered to be part of any motifs.

Now the problem left is how should we model this assignment matrix $\mC{(i)}$. We would like to include both the structural information and the features information in our model. Node embeddings from the GNN encoder $\bm E(\cdot)$ provides enough feature information of each node. We can apply a similar clustering procedure on the node level embeddings as we did for subgraphs in \ref{subsec:motif_learner}, so we generate node embeddings $\{\ve_1, ..., \ve_{N_i} \}$ of all $N_i$ nodes in $\gG_i$. Then we compute the cosine similarity between node and motif embeddings as $\emS_{j, k}^{(i)} = \phi(\ve_{j})^T\phi(\vm_{k})$. A further softmax normalization with temperature $\tau_s$ gives the result, $\mC_{j, k}^{(i)} = \frac{\exp(\emS_{j, k} / \tau_s)}{\sum_{k'}\exp(\emS_{j, k'} / \tau_s)}$. 


\paragraph{Training the Sampler}

After that we connect all $M$ assignment matrix to get the total $N = \sum_i N_i$ assignment, i.e. $\mS = \mid\mid \mS^{(i)}$. Then we follow the clustering loss in \ref{subsec:motif_learner} to use the Sinkhorn-Knopp algorithm to produce an optimal assignment $\mP$, as how we calculated $\mQ$ in equation \ref{eq: sinkhorn}. The loss function is thus the negative log likelihood as above.

\begin{equation} 
    {\cal L}_{n}  = -\frac{1}{N} \sum_{i=1}^{M}\sum_{j=1}^{N_i} \sum_{k = 1}^{K} \emP_{j, k} \log \emC_{j, k}^{(i)}
\end{equation}

The shortcoming of this approach is that the graph structure information is only used implicitly during the GNN message passing. This could result in an assignment rely too much on the feature information and assign node with the same feature to the same motif without looking at the structural difference. To capture the structural information more explicitly, we consider penalizing the difference between our clustering result and the result of spectral clustering. As spectral clustering performs really well in finding connected regions within a graph, the penalized loss will balance the feature and structural information. 

We show a regularization term proposed by Bianchi et al. \yrcite{bianchi2020spectral} in equation \ref{eq: mincut} . This regularization is a differentiable approximation of the spectral clustering. As Bianchi et al. mentioned in their paper, this regularizer term should be trained together with other task specific loss to find the optimal trade-off between task-specific and spectral clustering objectives, which is a perfect fit for our purpose. We refer readers to the paper for more discussion about how this loss server the role.

\begin{sequation}  \label{eq: mincut}
    {\cal L}_{r} \! = \!\frac{1}{M} \!\sum_{i = 1}^{M} \!-\frac{Tr(\mC^{(i) T}\!\mA^{(i)}\! \mC^{(i)})}{Tr(\mC^{(i)T}\!\mD^{(i)}\!\mC^{(i)})} + \bigg\Vert\frac{\hat\mC^{(i)T}\!\hat\mC^{(i)}}{\Vert\hat\mC^{(i)T}\!\hat\mC^{(i)}\Vert_{F}} - \frac{\mI_{J_i}}{\sqrt{J_i}}\bigg\Vert_{F}
\end{sequation}

% \begin{sequation}  \label{eq: mincut}
%     {\cal L}_{r} \! = \!\frac{1}{M} \!\sum_{i = 1}^{M} \!-\frac{Tr(\hat\mC^{(i) T}\!\mA^{(i)}\! \hat\mC^{(i)})}{Tr(\hat\mC^{(i)T}\!\mD^{(i)}\!\hat\mC^{(i)})} + \bigg\Vert\frac{\hat\mC^{(i)T}\!\hat\mC^{(i)}}{\Vert\hat\mC^{(i)T}\!\hat\mC^{(i)}\Vert_{F}} - \frac{\mI_{J_i}}{\sqrt{J_i}}\bigg\Vert_{F}
% \end{sequation}

% too long
% \begin{equation}  \label{eq: mincut}
%     {\cal L}_{spec}  = \frac{1}{M} \sum_{i = 1}^{M} -\frac{Tr(\hat\mC^{(i) T}\mA^{(i)} \hat\mC^{(i)})}{Tr(\hat\mC^{(i)T}\mD^{(i)}\hat\mC^{(i)})} + \bigg\Vert\frac{\hat\mC^{(i)T}\hat\mC^{(i)}}{\Vert\hat\mC^{(i)T}\hat\mC^{(i)}\Vert_{F}} - \frac{\mI_{J_i}}{\sqrt{J_i}}\bigg\Vert_{F}
% \end{equation}

where $||\cdot||_{F}$ denotes the Frobenius norm, $\mA^{(i)}$ is the adjacency matrix with self-loop, $\mD^{(i)}$ is the degree matrix of $\mA^{(i)}$, and $\hat\mC^{(i)}$ is the assignment matrix with only $J_i$ selected columns, i.e. only the motifs we are producing corresponding subgraphs.

Putting two terms together, the final loss for training the sampler is
\begin{equation}
    {\cal L}_s =  {\cal L}_{n} + {\cal L}_{r}
\end{equation}

% As this is just an regularization term, we won't let the regularization term dominate and the result matches exactly with the spectral clustering result.
% However, the spectral clustering requires eigen-decomposation, which is hard and slow. Therefore, we use the min-cut loss proposed in minCut pooling to approximate the spectral clustering. For more details about how to use this objective to approximate spectral clustering . Please refer to \cite{bianchi2020spectral}. 


% Our sampling strategy has two advantages over simple sampling strategies like random walk and k-hop neighbors. First, it generates samples utilizing both graph structure and feature information. This is because the sampling result depends on node representations, and the node representations contain both structure and feature information through the message passings in GNN. If the similarity score of a subgraph to the kth motif is higher than some threshold $\eta_k$, we use the following loss term to encourage nodes within this subgraph to become even similar to each other. 


% An example of subgraphs produced by our sampler after training can be found in Appendix \ref{appendix:sampler}


\subsection{Graph-to-subgraph Contrastive Learner} \label{subsec:contrastive}
Both the \textit{Motif Learner} and the \textit{Motif-guided sampler} rely on good (sub)graph embeddings. Therefore, an expressive GNN encoder $\bm E(\cdot)$ is essential for accurately identifying motifs. In our framework, we use contrastive learning to train the GNN encoder. Contrastive learning is one of the state-of-the-art self-supervised learning methods that achieves great results in vision and language domain. In contrastive learning, we generate positive view pairs from the same instance and make their representation simililar, and we generate negative view pairs form different instances and make their representations different.

More concretely, given a dataset with M graphs $\sG = \{\gG_{1}, ..., \gG_{M} \}$, $J_i$ subgraphs will be generated by the \textit{Motif-guided Sampler} from $\gG_{i}$. In total, there will be $J = \sum_{i=1}^{M} J_i$ subgraphs. We denote the embedding of these whole graphs and subgraphs as $\{\vh_1, ..., \vh_M\}$ and $\{\vs_1, ..., \vs_J\}$ respectively. Then we compute the graph-to-subgraph similarity matrix $\mY \in \R^{M \times J}$, where the entry $(i, j)$ is the cosine similarity between the corresponding graph-subgraph pair, i.e. $\emY_{i, j} = \phi(\vh_{i})^T \phi(\vs_{j})$. For the whole graph $\gG_i$, subgraphs sampled from it are considered as positive pairs to it, and subgraphs sampled from other graphs are considered as negative pairs to it. Then the contrastive objective function is the following, where we do row-wise softmax normalization with temperature parameter $\tau_c$ :
\begin{equation}
    {\cal L}_c  = -\frac{1}{M} \sum_{i=1}^{M} \sum_{j = 1}^{J}  \1\{g_j \in \gG_i\} \cdot \log \frac{\exp(\emY_{i, j} / \tau_c)}{\sum_{j'}\exp(\emY_{i, j'} / \tau_c)} 
\end{equation}

\begin{figure*}[h]
\begin{center}
\includegraphics[width=\textwidth]{picture/contrastive.png} 
\end{center}
\caption{ Different ways to generate views for graph data. Context Prediction uses one node and one context graph as views. InfoGraph uses one node and the whole graph as views. Our method uses a higher-level subgraph as one view and the whole graph as another; thus the GNN can capture more global contextual information. }
\label{figure:contrastive}
\end{figure*}

As shown in previous works, contrastive learning works more effectively when we can generate informative and diverse views of the data instances. Contrastive learning on graphs has been studied in \cite{hu2020pretraining, sun2019infograph}, but in both works at least one of the views is only node-level. Our method using graph-to-subgraph contrastive is better at capturing higher-level information then node-level contrastive. We show the different view generation strategy used in our model and previous work in \ref{figure:contrastive}. We discuss why we use graph-to-subgraph contrastive and other design choices in \ref{subsec:ablation}. Experiment results demonstrate the advantage of our approach.

\subsection{Joint training}
The whole framework of \textit{\method} can be trained jointly with a weighted sum of all three loss terms described above.
\begin{equation}
{\cal L} =  \lambda_m {\cal L}_m + \lambda_s {\cal L}_s + \lambda_c {\cal L}_c
\end{equation}

This objective allow us to simultaneously train an expressive GNN encoder and learn motifs from a given graph dataset. When the training starts, the motif embeddings are randomly initialized and the motif-like subgraphs are rather random. As the training goes, the motif learning and contrastive learning will mutually enhance each other and more accurately identify motifs. We visualize the the learned motifs in Figure \ref{figure:motif}. Pseudocode of our approach is shown in Algorithm \ref{algo:main}.


\begin{figure}[ht]
\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{picture/top_motifs.png}}
\caption{Top-6 frequently occurred motifs, represented by their closest subgraph.}
\label{figure:motif}
\end{center}
\vskip -0.2in
\end{figure}


% Pseudocode of our approach is shown in Algorithm \ref{algo:main}. First, we initialize the motif vectors and GNN encoder (line 2 - 3). For each batch of graphs $\sG = \{\gG_{i}\}_{i=1}^{B}$, the Sampler calculates the node-node affinity matrices $\mA^{(i)}$s and extract subgraphs based on the affinity scores (line 5 - 6). After that, GNN message passing is applied on whole graphs to get node embeddings, which are aggregate for both graph and subgraph embeddings (line 7 - 9). The next step is to compute the motif-to-subgraph similarity matrix $\mZ$. Using $\mZ$ we compute both the threshold $\eta$ and cluster assignment matrix $\mQ$ (line 11 - 13). With all these values, the three loss terms and the final joint loss introduced above can be computed (line 15 - 20).

\begin{algorithm}[h]
\lstset{style=style_snippet}
\begin{lstlisting}[language=Python]
# weight parameters: lamb_m, lamb_c, lamb_s
# projection parameters: W_e, W_h, W_s
# input a batch of whole graphs data = {G_1,..., G_M}
def __init__(args)
    self.encoder = GNN(args) # GNN encoder for pre-training
    self.motifs = nn.Parameters(K, embedding_dim) 
    
def forward(self, data)
    e, h = model.encoder(data) # e/h: node/graph embeddings
    adj = get_adj_matrix(data) # [A^{(1)},...,  A^{(M)}]
    
    # detach motifs and compute pairwise cosine sim
    C = cos_sim(torch.matmul(W_e, e), self.motifs.detach())
    with torch.no_grad(): 
        P = sinkhorn(C) # solve P using the Sinkhorn-Knopp
    
    #num_subs: number of subgraphs per graph [J_1,..., J_M] 
    s, num_subs = pool_subgraphs(e, P)
    
    loss_s = self.sampler_loss(P, C, adj)
    loss_m = self.motif_loss(s, P) # equation ()
    loss_c = self.contra_loss(h, s, num_subs) # equation ()    
    loss = lamb_s*loss_s + lamb_m*loss_m + lamb_c*loss_c
    return loss
    
def sampler_loss(self, P, C, adj):
    loss_node = -(P*log_softmax(C/tau_s, dim=1)).sum(dim=1)
    loss_spec = spectral_loss(C, adj) # equation ()
    loss_s = loss_node.mean() + loss_spec
    return loss_s

def motif_loss(self, s, P)
    # detach sub embeddings and compute pairwise cosine sim
    Z = cos_sim(torch.matmul(W_s, s.detach()), self.motifs)
    loss_m = -(P*log_softmax(Z/tau_m, dim=1)).sum(dim=1)    
    return loss_m.mean()

def contra_loss(self, h, s, num_subs):
    blocks = [torch.ones(1, int(n)) for n in num_subs]
    Y_lab = torch.block_diag(*blocks)
    Y = pairwise_cosine_sim(torch.matmul(W_h, h), s)
    loss_c = -(Y_lab*log_softmax(Y/tau_c, dim=1)).sum(dim=1)
    return loss_c.mean()
\end{lstlisting}
\caption{Pseudocode of MICRO-Graph in PyTorch Style, Full Version in Appendix \ref{appendix:code}}
\label{algo:main}
\end{algorithm}


% (For whether the graph-to-subgraph makes sense, please refer to \ref{figure:whole_motif_assign}, that different subgraphs will triger different dimensions of the whole graph.)

% Moreover, the motif learning and contrastive learning are mutually reinforced: a better GNN produces more accurate subgraph embeddings and thus help motif mining, while better motifs can help generate more informative graph-to-subgraph views and benefit contrastive learning.



==> section/_0_method_old3.tex <==

\begin{figure*}[h!]
\begin{center}
\includegraphics[width=\textwidth]{picture/framework.png} 
\end{center}
\caption{Overall framework of \textit{\method}. A GNN trained in a self-supervised manner to automatically extract motifs. The learned motifs are leveraged to generate informative subgraphs for graph-to-subgraph contrastive learning.}
\label{figure:framework}
\end{figure*}

\subsection{The Overall Framework of \textit{\method}} \label{subsec:framework}
Graph motif discovery through exact counting is a combinatorial problem, which is hard to generalize to large datasets with continuous or high-dimensional features. We propose to turn the motif learning problem from discrete to differentialble using embedding vectors encoded by GNNs. 

% Our goal is to train a GNN encoder via contrastive learning to generate meaningful (sub)graph level representations, based on which to extract graph motifs. The learned motifs can reversely benefit the contrastive learning.

Given a dataset, our goal is to learn two things:
1) A GNN-based graph encoder $\bm {ENC}_{\theta}(\cdot)$ that maps input (sub)graphs to D-dimensional embedding vectors that captures their semantic properties.
2) A $K$-slot motif embedding table $\{\vm_{1}, ..., \vm_{K}\}$, where each slot stores a prototypical D-dimensional embedding. These $K$ embedding are our motif embedding vectors, which represents semantic properties shared by many subgraph patterns.


% This is more useful abstraction because people study exact patterns for their semantic meanings. 
% It used to be that case that two subgraph patterns differ by a little are considered different motifs, but in our framework they could correspond to the same motif embedding because they share very similar semantic meanings. 

% This is especially useful because some structurally similar graphs can deliver very different properties.


% An example from chemistry would be a sulfate ($-SO_4$) and a phosphate ($-PO_4$). Although these two functional groups don't match exactly, they are considered to be the same motif in our sense and they indeed share very similar chemical properties. 


The \textit{\method} framework learn these two things through two modules
% for solving the two research questions we mentioned in the Introduction.
\begin{compactitem}
    \item A \textit{Motif-Learner} to group nodes to motif-like subgraphs and learn motif embeddings by maximizing the likelihood of the subgraph embeddings.
    % extract graph motifs by clustering these subgraphs.
    \item A contrastive learning module leveraging graph motifs to generate more informative view for training the GNN encoder $\bm {ENC}_{\theta}(\cdot)$.
    % self-supervised GNN-based representation learning.
\end{compactitem}

The overall framework is shown in Figure\ref{figure:framework}. We describe the details of these two modules in order in the following sections. (go over framework)


\subsection{Motif Learner via an EM Algorithm}\label{subsec:motif_learner}
We first describe how does the \textit{Motif Learner} module learn motif embeddings via an EM algorithm. 


I think you should give a brief overview what each part is saying. For example, the first part is about generate motif-like subgraph. In this part, you model the probability of each node belonging to each motif, and you do xxx. The second part is update motif embedding, where you group subgraphs and get subgraph embdding. (2) Right now it's ""super"" unclear what each part is doing. Just give a overview at beginging before introducing the details.


In the E-step, we would like to group nodes to form motif-like subgraphs which have high probability belonging to a specific motif. In the M-step, we would like to update the motif embeddings by maximizing the log-likelihood that the corresponding motif contains these motif-like subgraphs. 


Given a dataset with $M$ graphs $\sG = \{\gG_{1}, ..., \gG_{M} \}$, for each $\gG_{i}$ in $\sG$, we denote its $N_i$ nodes by $\{n_{1}^{(i)}, ..., n_{N_i}^{(i)} \}$ and their corresponding embeddings by $\{\ve_{1}^{(i)}, ..., \ve_{N_i}^{(i)}\} = \bm {ENC}_{\theta}(\gG_i)$. We would like to group these nodes into $J_i$ subgraphs denoted as $\{g_{1}^{(i)}, ..., g_{J_i}^{(i)} \}$ and their corresponding embeddings as $\{\vs_{1}^{(i)}, ..., \vs_{J_i}^{(i)}\}$. For each subgraph $g_{j}^{(i)}$, we use a K-way categorical random variable $Z_j^{(i)}$ to denote which motif this subgraph belongs.
\begin{equation}
    P(Z_j^{(i)} = k) = P(\vs_{j}^{(i)} \sim \vm_k), \text{ for } 1 \leq k \leq K
\end{equation}

We would like to group nodes to motif-like subgraphs. At the node level, we use another K-way categorical random variables $C_l^{(i)}$ to denote which motif a subgraph formed by this node should belongs to.
\begin{align}
    P(C_l^{(i)} = k) = \sum_j P(n_{l}^{(i)} \in g_{j}^{(i)} \text{ and } \vs_{j}^{(i)} \sim \vm_k), \\
    \text{ for } 1 \leq k \leq K \nonumber
\end{align}

Here we slightly abuse notation to use $\sim$ between embeddings to denote the ``belongs to".

% Here we slightly abuse notation to use $\in$ and $\sim$ between embeddings to denote the ``belongs to" and ``similar to". We will discuss in the M-step about how to use $\ve_{l}^{(i)}$, $\vs_{j}^{(i)}$, and $\vm_k$ to model these two relationships exactly.

We model $Z^{(i)}$  as pairwise cosine similarities between subgraph embeddings and motif embeddings, followed by a softmax normalization to turn values probabilities.
\begin{equation} \label{equation:sub_motif}
P(Z_j^{(i)} = k) = \frac{\exp(\phi(W_s \vs_{j}^{(i)})^T\phi(\vm_{k}) / \tau_s)}{\sum_{j'}\exp(\phi(W_s \vs_{j'}^{(i)})^T\phi(\vm_{k}) / \tau_s)}
\end{equation}

Here we use $\phi(x) = x \ / \ \Vert x \Vert_{2}$ to denote the L-2 normalization, and $\tau_s$ is a temperature parameter. Also, we project $\vs_{j}^{(i)}$ with a projection parameter matrix $W_s$ in order to capture the asymmetric ``belongs to" relationship.

We model $C^{(i)}$ in a similar way,
\begin{equation} \label{equation:node_motif}
P(C_l^{(i)} = k) = \frac{\exp(\phi(W_e \ve_{l}^{(i)})^T\phi(\vm_{k}) / \tau_n)}{\sum_{l'}\exp(\phi(W_e \ve_{l'}^{(i)})^T\phi(\vm_{k}) / \tau_n)}
\end{equation}
The difference is that we use different temperature and projection parameters $\tau_n$ and $W_n$.


\textbf{E-Step}. In the E-step, we assume we have all the embeddings $\ve_{l}^{(i)}$, $\vs_{j}^{(i)}$, and $\vm_k$, and thus the current estimates of the distributions of $C_l^{(i)}$ and $Z_j^{(i)}$. We will based on them to figure out optimal node-to-motif assignments and subgraph-to-motif assignments.

Given a graph $\gG_i$, we denote the node-to-motif assignments as $\mQ^{(i)} \in \{0,1\}^{N_i \times K} $. Here the $l$th row $\mQ^{(i)}_l$ is an one-hot vector represents which motif $n_l^{(i)}$ is assigned to, i.e. $\sum_{k} \mQ^{(i)}_{l,k} = 1, \forall 1 \leq l \leq N_i$.  $\mQ^{(i)}$ will be used to sample motif-like subgraphs from $\gG_i$ by taking the induced subgraph of nodes assigned to the same motif. In other words, for each column $k$ of $\mQ^{(i)}$, if $\{n_l \vert \mQ^{(i)}_{l, k} = 1\} \neq \emptyset$, we generate an induced subgraph with these nodes.\footnote{In practice, instead of considering all nonempty node sets, we can set a threshold $\eta$ and only consider $|\{n_l \vert \mQ^{(i)}_{l, k} = 1\} | > \eta$ to filter out small subgraphs.} When sampling from $M$ input graphs, we denote the assignments of all $N = \sum_{i=1}^M N_i$ nodes as $\mQ = [\mQ^{(1)}, ..., \mQ^{(M)}]$. 

The optimal assignment $\mQ^*$ is the one that maximizes the joint probability of all $C_{l}^{(i)}$'s. This $\mQ^*$ guarantees each generated subgraph will likely to be similar to a particular motif, since all the nodes in it have high probability being part of that motif. Formally, this can be written as a constrained optimization problem in \ref{equation:vanilla}, where $\mC = [C_1^{(1)}, ..., C_{N_1}^{(1)}, C_{1}^{(2)}, ..., C_{N_M}^{(M)}]^T$ denotes all $N \times K$ node-to-motif probabilities.
\begin{gather} \label{equation:vanilla}
\mQ^* = \argmax_{\mQ} Tr(\mQ\mC^T)\\
\text{s.t. } \mQ \in \{0, 1\}^{N \times K} \text{ and } \sum_{k} \mQ_{l,k} = 1, \forall 1 \leq l \leq N \nonumber
\end{gather}
This objective works fine for the E-step along. However, it is problematic when we do the joint training with the representation learning in the M-step. Each time we run the M-step, the node embeddings $\ve_{l}^{(i)}$ will change due to the GNN parameters update. Therefore, there exists a degenerate solution for this vanilla objective, which is all embeddings collapse together and thus got assigned to the same motif. Similar issues were observed in previous works when doing representation learning and assignment estimation together \cite{asano2020self, caron2020unsupervised}. To avoid this issue, we adopt the strategy used in \cite{asano2020self} to approximate $\mQ^*$ by solving a slightly modified optimization problem. The modifications include adding an entropy term $H(\bm{Q}) = - \sum_{l,k}\mQ_{l,k} \log \mQ_{l,k}$ to the objective and change the searching space of $\mQ$ to the following:
% the constraint set $\cal Q$ requires the marginal projection of $\bm Q$ onto its columns and rows to be uniform.
\begin{equation}
    {\cal Q} = \{\bm{Q} \in \mathbb{R}_+^{N, K} | \bm{Q 1_{K}} = \frac{\bm{1_N}}{N}, \bm{Q^T 1_{N}} = \frac{\bm{1_K}}{K} \} 
\end{equation}
where $\bm{1_{N}}$ and $\bm{1_{K}}$ are all one vectors. 

Therefore, the final objective thus becomes the following with $\lambda$ being a hyper-parameter. In practice, it will be set to some large number so the influence of $H(\bm{Q})$ is negligible.
\begin{equation}
    \max_{\bm Q \in \cal{Q}} Tr(\bm{Q} \mC^T) + \frac{1}{\lambda} H(\bm{Q})
\end{equation}
For more reasons about why this new objective can help avoid the degenerate solution and why it gives a reasonable approximation of $\mQ^*$, we refer the readers to \cite{asano2020self}. Here we will only mention one good property that motivates us to choose this modified optimization problem, which is this problem has a closed-form solution showing in (\ref{eq: sinkhorn}).
\begin{equation} \label{eq: sinkhorn}
    \mQ  = Diag(\vu) \cdot \exp(\lambda \mC) \cdot Diag(\vv)
\end{equation}
Here $\bm u$ and $\bm v$ are merely normalization vectors to make sure $\mQ$ is a probability matrix. These two parameters can be solved efficiently using a fast Sinkhorn-Knopp algorithm as shown in \cite{cuturi2013sinkhorn}. The probability matrix can be turned into a hard assignment matrix by simply taking row-wise argmax.

The last thing of the E-step is to compute the subgraph-to-motif assignments for all $J = \sum_{i=1}^{M} J_i$ subgraphs, which we denote as $\mP = [\mP^{(1)}, ..., \mP^{(M)}] \in \{0, 1\}^{J \times K}$. As we already know the node-to-motif assignments $\mQ$, and by our sampling procedure all nodes within the same subgraph will have the same assignment, we simply make the motif assignment of any subgraph the same as the motif assignment of any node in the subgraph, i.e. $\mP_{j, k}^{(i)} = \mQ_{l, k}^{(i)}, \forall n_l^{(i)} \in g_j^{(i)}$.


\paragraph{M-Step} 
The goal of the M-step is to learn the parameters in $P(C_l^{(i)} = k)$ and $P(Z_j^{(i)} = k)$ by maximizing the log-likelihood of the data given the assignment matrix $\mQ$ and $\mP$ computed in the E-step. As we mentioned above, $P(C_l^{(i)} = k)$ and $P(Z_j^{(i)} = k)$ are modeled using the embeddings $\ve_{l}^{(i)}$, $\vs_{j}^{(i)}$, and $\vm_k$. Thus, when maximizing the log-likelihood, we also update parameters in the GNN encoder and the motif embedding table. 

The negative log-likelihood losses are thus 
\begin{align}
{\cal L}_{sample} = -\frac{1}{N} \sum_{i=1}^{M} \sum_{l=1}^{N_i} \sum_{k = 1}^{K} \mQ_{l, k}^{(i)} \log P(C_l^{(i)} = k) \\
{\cal L}_{motif} = -\frac{1}{J} \sum_{i=1}^{M}\sum_{j=1}^{J_i} \sum_{k = 1}^{K} \mP_{j, k}^{(i)} \log P(Z_j^{(i)} = k)
\end{align} 

% We use gradient to update the GNN parameters and motif embeddings. 
As all the procedures are differentiable, we can use standard gradient-based optimizer to update the GNN parameters and motif embeddings. 
Notice that the ${\cal L}_{sample}$ is only used to train the model to generate motif-like subgraph, so during gradient descent we won't use its gradient to update the motif embeddings. On the other hand, ${\cal L}_{motif}$ is used for motif embedding learning, so during gradient descent we won't use its gradient to update the node/subgraph embeddings. Thus, all the parameters we would like to update will only get gradient from one of these two losses, even some are used in the calculation of both equation \ref{equation:node_motif} and \ref{equation:sub_motif}.


The final notice is that when modeling $\mC^{(i)}$ in equation \ref{equation:node_motif}, the graph structure information is only used implicitly by generating node embeddings using the GNN message passing. This could result in an assignment rely too much on the feature information and assign node with the similar feature to the same motif without looking at the structural difference. To capture the structural information more explicitly, we include another spectral clustering based regularization term ${\cal L}_{r}$ proposed by Bianchi et al. \yrcite{bianchi2020spectral}. This term makes our assignment $\mQ$ close to the result of spectral clustering, and penalizes nodes that are too far away to be assigned to the same motif, and thus balances the usage of feature and structural information in motif-like subgraph generation.


% We show a regularization term proposed by Bianchi et al. \yrcite{bianchi2020spectral} in equation \ref{eq: mincut} . This regularization is a differentiable approximation of the spectral clustering. As Bianchi et al. mentioned in their paper, this regularizer term should be trained together with other task specific loss to find the optimal trade-off between task-specific and spectral clustering objectives, which is a perfect fit for our purpose.
% We refer readers to the paper for more discussion about how this loss server the role.

\begin{sequation}  \label{eq: mincut}
    {\cal L}_{r} \! = \!\frac{1}{M} \!\sum_{i = 1}^{M} \!-\frac{Tr(\mC^{(i) T}\!\mA^{(i)}\! \mC^{(i)})}{Tr(\mC^{(i)T}\!\mD^{(i)}\!\mC^{(i)})} + \bigg\Vert\frac{\hat\mC^{(i)T}\!\hat\mC^{(i)}}{\Vert\hat\mC^{(i)T}\!\hat\mC^{(i)}\Vert_{F}} - \frac{\mI_{J_i}}{\sqrt{J_i}}\bigg\Vert_{F}
\end{sequation}


In equation \ref{eq: mincut}, $||\cdot||_{F}$ denotes the Frobenius norm, $\mA^{(i)}$ is the adjacency matrix with self-loop of $\gG_i$, $\mD^{(i)}$ is the degree matrix of $\mA^{(i)}$, and $\hat\mC^{(i)}$ is the assignment matrix with only $J_i$ selected columns, i.e. only the motifs we are producing corresponding subgraphs.

\paragraph{Comparison with Existing Motif Mining methods}
Different from the traditional motif that only considers structural patterns, the motif embeddings in our framework can group structurally-dissimilar subgraphs that share similar semantic meanings into a motif slot.
% This is more useful abstraction because people study exact patterns for their semantic meanings. 
% It used to be that case that two subgraph patterns differ by a little are considered different motifs, but in our framework they could correspond to the same motif embedding because they share very similar semantic meanings. 
% This is especially useful because some structurally similar graphs can deliver very different properties.
An example from chemistry would be a sulfate ($-SO_4$) and a phosphate ($-PO_4$). Although these two functional groups don't match exactly, they are considered to be the same motif in our sense and they indeed share very similar chemical properties. 

% As this is just an regularization term, we won't let the regularization term dominate and the result matches exactly with the spectral clustering result.
% However, the spectral clustering requires eigen-decomposation, which is hard and slow. Therefore, we use the min-cut loss proposed in minCut pooling to approximate the spectral clustering. For more details about how to use this objective to approximate spectral clustering . Please refer to \cite{bianchi2020spectral}. 


% Our sampling strategy has two advantages over simple sampling strategies like random walk and k-hop neighbors. First, it generates samples utilizing both graph structure and feature information. This is because the sampling result depends on node representations, and the node representations contain both structure and feature information through the message passings in GNN. If the similarity score of a subgraph to the kth motif is higher than some threshold $\eta_k$, we use the following loss term to encourage nodes within this subgraph to become even similar to each other. 


% An example of subgraphs produced by our sampler after training can be found in Appendix \ref{appendix:sampler}


\subsection{Motif-guided Contrastive Learning} \label{subsec:contrastive}
The \textit{Motif Learner} relies on good (sub)graph embeddings. Therefore, an expressive GNN encoder $\bm E(\cdot)$ is essential for accurately identifying motifs. In our framework, we use contrastive learning to train the GNN encoder. Contrastive learning is one of the state-of-the-art self-supervised learning methods that achieves great results in vision and language domain. In contrastive learning, we generate positive view pairs from the same instance and make their representation simililar, and we generate negative view pairs form different instances and make their representations different.

More concretely, we denote the graph embeddings of $\sG = \{\gG_{1}, ..., \gG_{M} \}$ as $\{\vh_1, ..., \vh_M\}$. Then we compute the graph-to-subgraph similarity matrix $\mY \in \R^{M \times J}$, where the entry $(i, j)$ is the cosine similarity between the corresponding graph-subgraph pair, i.e. $\mY_{i, j} = \phi(W_h \vh_{i})^T \phi(\vs_{j})$, where $W_h$ is a projection parameter matrix. For the whole graph $\gG_i$, subgraphs sampled from it are considered as positive pairs to it, and subgraphs sampled from other graphs are considered as negative pairs to it. Then the contrastive objective function is the following, where we do row-wise softmax normalization with temperature parameter $\tau_c$ :
\begin{sequation}
    {\cal L}_{contra}  = -\frac{1}{M} \sum_{i=1}^{M} \sum_{j = 1}^{J}  \1\{g_j \in \gG_i\} \cdot \log \frac{\exp(\mY_{i, j} / \tau_c)}{\sum_{j'}\exp(\mY_{i, j'} / \tau_c)} 
\end{sequation}
As shown in previous works, contrastive learning works more effectively when we can generate informative and diverse views of the data instances. Contrastive learning on graphs has been studied in \cite{hu2020pretraining, sun2019infograph}, but in both works at least one of the views is only node-level. Our method using graph-to-subgraph contrastive is better at capturing higher-level information then node-level contrastive. We show the different view generation strategy used in our model and previous work in \ref{figure:contrastive}. We discuss why we use graph-to-subgraph contrastive and other design choices in \ref{subsec:ablation}. Experiment results demonstrate the advantage of our approach.

\begin{figure*}[h]
\begin{center}
\includegraphics[width=\textwidth]{picture/contrastive.png} 
\end{center}
\caption{ Different ways to generate views for graph data. Context Prediction uses one node and one context graph as views. InfoGraph uses one node and the whole graph as views. Our method uses a higher-level subgraph as one view and the whole graph as another; thus the GNN can capture more global contextual information. }
\label{figure:contrastive}
\end{figure*}

\subsection{MICRO-Graph Objective}
The whole framework of \textit{\method} can be trained jointly with a weighted sum of all the loss terms described above.
\begin{equation}
{\cal L} =  \lambda_m {\cal L}_{motif} + \lambda_s {\cal L}_{sample} + \lambda_r {\cal L}_r + \lambda_c {\cal L}_{contra}
\end{equation}

This objective allow us to simultaneously train an expressive GNN encoder and learn motifs from a given graph dataset. When the training starts, the motif embeddings are randomly initialized and the motif-like subgraphs are rather random. As the training goes, the motif learning and contrastive learning will mutually enhance each other and more accurately identify motifs. We visualize the the learned motifs in Figure \ref{figure:motif}. Pseudocode of our approach is shown in Algorithm \ref{algo:main}.


\begin{figure}[ht]
\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{picture/top_motifs.png}}
\caption{Top-6 frequently occurred motifs, represented by their closest subgraph.}
\label{figure:motif}
\end{center}
\vskip -0.2in
\end{figure}


\begin{algorithm}[h]
\lstset{style=style_snippet}
\begin{lstlisting}[language=Python]
# weight parameters: lamb_m, lamb_c, lamb_s, lamb_r
# projection parameters: W_e, W_h, W_s
# input a batch of whole graphs data = {G_1,..., G_M}
def __init__(args)
    self.encoder = GNN(args) # GNN encoder for pre-training
    self.motifs = nn.Parameters(K, embedding_dim) 
    
def forward(self, data)
    e, h = model.encoder(data) # e/h: node/graph embeddings
    adj = get_adj_matrix(data) # [A^{(1)},...,  A^{(M)}]
    
    # detach motifs and compute pairwise cosine sim
    C = cos_sim(torch.matmul(W_e, e), self.motifs.detach())
    C = softmax(C/tau_s, dim=1)
    with torch.no_grad(): 
        Q = sinkhorn(C) # solve Q using the Sinkhorn-Knopp
    
    #num_subs: number of subgraphs per graph [J_1,..., J_M] 
    s, P, num_subs = pool_subgraphs(e, Q)
    
    l_s, l_r = self.sample_loss(Q, C, adj) # equation (9)
    l_m = self.motif_loss(s, P) # equation (10)
    l_c = self.contra_loss(h, s, num_subs) #equation(12)    
    loss = lamb_s*l_s + lamb_m*l_m + lamb_c*l_c + lamb_r*l_r
    return loss
    
def sample_loss(self, Q, C, adj):
    loss_sample = -(Q * C.log()).mean().sum(dim=1)
    loss_r = spectral_loss(C, adj) # equation (11)
    return loss_sample, loss_r

def motif_loss(self, s, P)
    # detach sub embeddings and compute pairwise cosine sim
    Z = cos_sim(torch.matmul(W_s, s.detach()), self.motifs)
    Z = softmax(Z / tau_m, dim=1)
    loss_motif = -(P * Z.log()).sum(dim=1).mean()   
    return loss_motif

def contra_loss(self, h, s, num_subs):
    blocks = [torch.ones(1, int(n)) for n in num_subs]
    Y_lab = torch.block_diag(*blocks)
    Y = pairwise_cosine_sim(torch.matmul(W_h, h), s)
    loss_contra = - (Y_lab * log_softmax(Y/tau_c, dim=1))
    return loss_contra.sum(dim=1).mean()
\end{lstlisting}
\caption{Pseudocode of MICRO-Graph in PyTorch Style, Full Version in Appendix \ref{appendix:code}}
\label{algo:main}
\end{algorithm}


% (For whether the graph-to-subgraph makes sense, please refer to \ref{figure:whole_motif_assign}, that different subgraphs will triger different dimensions of the whole graph.)

% Moreover, the motif learning and contrastive learning are mutually reinforced: a better GNN produces more accurate subgraph embeddings and thus help motif mining, while better motifs can help generate more informative graph-to-subgraph views and benefit contrastive learning.





==> section/allTables.tex <==
All the tables in the experiment section

\begin{table}[h]
\center
\scalebox{0.68}{
\begin{tabular}{@{}l|ccccccc|c@{}}
\toprule
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}c@{}} SSL methods \end{tabular}} & \multicolumn{1}{c}{bace} & bbbp & clintox & hiv & sider & tox21 & toxcast & Average\\ \midrule
Non-Pretrain & 72.80 $\pm$ 2.12 & 82.13 $\pm$ 1.69 & 74.98 $\pm$ 3.59 & 73.38 $\pm$ 0.92 & 55.65 $\pm$ 1.35 & 76.10 $\pm$ 0.58 & 63.34 $\pm$ 0.75  & 71.19\\ \midrule
ContextPred & 73.02 $\pm$ 2.59 & 80.94 $\pm$ 2.55 & 74.57 $\pm$ 3.05 & 73.85 $\pm$ 1.38 & 54.15 $\pm$ 1.54 & 74.85 $\pm$ 1.28 & 63.19 $\pm$ 0.94  & 70.65 (\ -0.7\%)\\
InfoGraph & 76.09 $\pm$ 1.63 & 80.38 $\pm$ 1.19 & \textbf{78.36 $\pm$ 4.04} & 72.59 $\pm$ 0.97 & 56.88 $\pm$ 1.80 & 76.12 $\pm$ 1.11 & 64.40 $\pm$ 0.84 & 72.11 (+1.3\%)\\
GPT-GNN & 75.56 $\pm$ 2.49 & 83.35 $\pm$ 1.70 & 74.84 $\pm$ 3.45 & 74.82 $\pm$ 0.99 & 55.59 $\pm$ 1.58 & 76.34 $\pm$ 0.68 & 64.76 $\pm$ 0.62 & 72.18 (+1.4\%)\\
% DGI & \textbf{76.59 $\pm$ 2.45} & 83.46 $\pm$ 1.75 & 74.8 $\pm$ 2.38 & 75.15 $\pm$ 1.24 & 56.9 $\pm$ 1.19 & 76.59 $\pm$ 0.61 & 65.27 $\pm$ 0.62 \\
\midrule
\itextit{\method} & \textbf{76.16 $\pm$ 2.51} & \textbf{83.78 $\pm$ 1.77} & 77.50 $\pm$ 3.35 & \textbf{75.51 $\pm$ 0.67} & \textbf{57.28 $\pm$ 1.09} & \textbf{76.68 $\pm$ 0.36} & \textbf{65.42 $\pm$ 0.62} & \textbf{73.19 (+2.8\%)}\\
\bottomrule
\end{tabular}}
\caption{HIV, Finetune, ROC, CV 0.1}
\end{table}



\begin{table}[h]
\center
\scalebox{0.72}{
\begin{tabular}{@{}l|ccccccc|c@{}}
\toprule
\multicolumn{1}{l|}{\begin{tabular}[l]{@{}c@{}}SSL methods\end{tabular}} & \multicolumn{1}{c}{bace} & bbbp & clintox & hiv & sider & tox21 & toxcast  & Average\\ \midrule
% Non-Pretrain & \\ 
% \midrule
ContextPred & 53.09 $\pm$ 0.84 & 55.51 $\pm$ 0.08 & 40.73 $\pm$ 0.02 & 53.31 $\pm$ 0.15 & 52.28 $\pm$ 0.08 & 35.31 $\pm$ 0.25 & 47.06 $\pm$ 0.06 & 48.18 \\
InfoGraph & 66.06 $\pm$ 0.82 & 75.34 $\pm$ 0.51 & \textbf{75.71 $\pm$ 0.53} & 61.45 $\pm$ 0.74 & 54.7 $\pm$ 0.24 & 63.95 $\pm$ 0.24 & 52.69 $\pm$ 0.07 & 64.27 \\
GPT-GNN & 59.43 $\pm$ 0.66  & 71.58 $\pm$ 0.54 & 62.78 $\pm$ 0.58 & 64.08 $\pm$ 0.36 & 54.67 $\pm$ 0.16 & 68.2 $\pm$ 0.14 & 57.06 $\pm$ 0.13 & \textbf{62.53}\\
% DGI & \\ 
\midrule
\method & \textbf{69.54 $\pm$ 0.39} & \textbf{81.07 $\pm$ 0.42} & 63.69 $\pm$ 0.56 & \textbf{72.74 $\pm$ 0.15} & \textbf{55.39 $\pm$ 0.26} & \textbf{72.91 $\pm$ 0.12} & \textbf{61.04 $\pm$ 0.07} & \textbf{68.05}\\
\bottomrule
\end{tabular}
}
\caption{HIV, Linear, ROC, CV 0.1, last-layer}
\end{table}



\begin{table}[!h]
\center
\scalebox{0.69}{
\begin{tabular}{@{}l|ccccccc|c@{}}
\toprule
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}c@{}} SSL methods \end{tabular}} & \multicolumn{1}{c}{bace} & bbbp & clintox & hiv & sider & tox21 & toxcast & Average\\ \midrule
Non-Pretrain & 72.80 $\pm$ 2.12 & 82.13 $\pm$ 1.69 & 74.98 $\pm$ 3.59 & 73.38 $\pm$ 0.92 & 55.65 $\pm$ 1.35 & 76.10 $\pm$ 0.58 & 63.34 $\pm$ 0.75  & 71.19\\ 
\midrule
ContextPred & 78.2 $\pm$ 2.04 & 81.52 $\pm$ 2 & 67.05 $\pm$ 3.49 & 75.59 $\pm$ 0.94 & 56.26 $\pm$ 1.26 & 75.14 $\pm$ 0.85 & 64.31 $\pm$ 0.66 & 71.15\\
InfoGraph & 76.27 $\pm$ 2.23 & 82.93 $\pm$ 1.87 & 77.72 $\pm$ 2.73 & 72.63 $\pm$ 1.42 & 56.64 $\pm$ 1.5 & 75.38 $\pm$ 0.97 & 63.92 $\pm$ 1.1 & 72.21 \\
GPT-GNN & 76.02 $\pm$ 2.26 & 83.03 $\pm$ 1.94 & 73.66 $\pm$ 3.08 & 74.82 $\pm$ 1.08 & 55.19 $\pm$ 1.25 & 76.2 $\pm$ 0.68 & 64.63 $\pm$ 0.78 & 71.93\\
DGI & 73.88 $\pm$ 2.81 & 81.86 $\pm$ 2.08 & 72.16 $\pm$ 2.75 & 74.41 $\pm$ 1.04 & 55.85 $\pm$ 1.72 & 76.06 $\pm$ 0.55 & 64.55 $\pm$ 0.57 & 71.25\\ \midrule
\method & 77.64 $\pm$ 2.29 & 83.25 $\pm$ 1.56 & 77.47 $\pm$ 3.24 & 75.62 $\pm$ 0.63 & 57.01 $\pm$ 1.93 & 76.99 $\pm$ 0.66 & 65.52 $\pm$ 0.65 & 73.36 (+2.17)\\
\bottomrule
\end{tabular}}
\caption{Zinc, Finetune, ROC, CV 0.1}
\end{table}


\begin{table}[!h]
\center
\scalebox{0.72}{
\begin{tabular}{@{}l|ccccccc|c@{}}
\toprule
\multicolumn{1}{l|}{\begin{tabular}[l]{@{}c@{}}SSL methods\end{tabular}} & \multicolumn{1}{c}{bace} & bbbp & clintox & hiv & sider & tox21 & toxcast  & Average\\ \midrule
% Non-Pretrain & \\ 
% \midrule
ContextPred & \\
InfoGraph & \\
GPT-GNN & \\
% DGI & \\ 
\midrule
\method & \\
\bottomrule
\end{tabular}
}
\caption{Zinc, Linear, ROC, CV 0.1, last-layer}
\end{table}


\begin{table}[h]
\center
\scalebox{0.69}{
\begin{tabular}{@{}l|ccccccc|c@{}}
\toprule
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}c@{}} SSL methods \end{tabular}} & \multicolumn{1}{c}{bace} & bbbp & clintox & hiv & sider & tox21 & toxcast & Average\\ \midrule
Non-Pretrain & 72.80 $\pm$ 2.12 & 82.13 $\pm$ 1.69 & 74.98 $\pm$ 3.59 & 73.38 $\pm$ 0.92 & 55.65 $\pm$ 1.35 & 76.10 $\pm$ 0.58 & 63.34 $\pm$ 0.75  & 71.19\\ \midrule
\midrule
\itextit{\method} & \\
\bottomrule
\end{tabular}}
\caption{HIV, Finetune, ROC, CV 0.1, GIN}
\end{table}


==> section/deprecatedTables.tex <==
Deprecated tables in the experiment section

\begin{table}[!h]
\center
\scalebox{0.72}{
\begin{tabular}{@{}l|ccccccc|c@{}}
\toprule
\multicolumn{1}{l|}{\begin{tabular}[l]{@{}c@{}}SSL methods\end{tabular}} & \multicolumn{1}{c}{bace} & bbbp & clintox & hiv & sider & tox21 & toxcast  & Average\\ \midrule
% Non-Pretrain & \\ 
% \midrule
ContextPred & 59.64 $\pm$ 0.31 & 66.69 $\pm$ 0.38 & 39.28 $\pm$ 0.8 & 61.67 $\pm$ 0.35 & 52.4 $\pm$ 0.45 & 49.78 $\pm$ 0.43 & 50.15 $\pm$ 0.18 & 54.23\\
InfoGraph & 76.03 $\pm$ 0.32 & 84.15 $\pm$ 0.46 & \textbf{84.61 $\pm$ 0.54} & 70.47 $\pm$ 0.93 & 58.17 $\pm$ 0.31 & 72.83 $\pm$ 0.15 & 61.2 $\pm$ 0.08 & 72.49\\
GPT-GNN & 65.58 $\pm$ 0.24 & 78.77 $\pm$ 0.12 & 71.83 $\pm$ 0.71 & 70.4 $\pm$ 0.06 & 58.25 $\pm$ 0.24 & 74.15 $\pm$ 0.08 & 63.91 $\pm$ 0.06 & 68.98\\
% DGI & \\ 
\midrule
\method & \textbf{79.95 $\pm$ 0.17} & \textbf{85.86 $\pm$ 0.18} & 77.83 $\pm$ 0.89 & \textbf{75.92 $\pm$ 0.08} & \textbf{62.48 $\pm$ 0.3} & \textbf{78.47 $\pm$ 0.15} & \textbf{67.42 $\pm$ 0.04} & 75.42\\
\bottomrule
\end{tabular}
}
\caption{HIV, Linear, ROC, CV 0.9 , last-layer}
\end{table}

\begin{table}[!h]
\center
\scalebox{0.72}{
\begin{tabular}{@{}l|ccccccc|c@{}}
\toprule
\multicolumn{1}{l|}{\begin{tabular}[l]{@{}c@{}}SSL methods\end{tabular}} & \multicolumn{1}{c}{bace} & bbbp & clintox & hiv & sider & tox21 & toxcast  & Average\\ \midrule
% Non-Pretrain & \\ 
% \midrule
ContextPred & 58.96 $\pm$ 0.18 & 68.66 $\pm$ 0.39 & 39.28 $\pm$ 0.8 & 61.94 $\pm$ 0.29 & 52.71 0.4 & 51.53 $\pm$ 0.37 & 50.66 $\pm$ 0.21\\
InfoGraph &  \\
GPT-GNN & \\
% DGI & \\ 
\midrule
\method & \textbf{79.95 $\pm$ 0.17} & \textbf{85.86 $\pm$ 0.18} & 77.83 $\pm$ 0.89 & \textbf{75.92 $\pm$ 0.08} & \textbf{62.48 $\pm$ 0.3} & \textbf{78.47 $\pm$ 0.15} & \textbf{67.42 $\pm$ 0.04}\\
\bottomrule
\end{tabular}
}
\caption{HIV, Linear, ROC, CV 0.9, penultimate layer}
\label{tab:linear}
\end{table}

\begin{table}[!h]
\center
\scalebox{0.72}{
\begin{tabular}{@{}l|ccccccc|c@{}}
\toprule
\multicolumn{1}{l|}{\begin{tabular}[l]{@{}c@{}}SSL methods\end{tabular}} & \multicolumn{1}{c}{bace} & bbbp & clintox & hiv & sider & tox21 & toxcast  & Average\\ \midrule
% Non-Pretrain & 69.09 $\pm$ 0.21 & 83.25 $\pm$  0.07 & 92.98 $\pm$ 0.00 & 96.49 $\pm$  0.00 & 75.71 $\pm$  0.04 & 92.40 $\pm$ 0.00 & 83.58 $\pm$ 0.00 & 84.78\\ 
% \midrule
ContextPred & 57.13 $\pm$ 0.55 & 80.58 $\pm$ 0.21 & \textbf{93.03 $\pm$ 0.00} & \textbf{96.49 $\pm$ 0.00} & 75.35 $\pm$ 0.08 & 92.21 $\pm$ 0.01 & 83.68 $\pm$ 0.02 & 82.64 \\
InfoGraph & 67.51 $\pm$ 1.83 & 82.08 $\pm$ 1.13 & 90.92 $\pm$ 0.40 & 93.24 $\pm$ 1.92 & 68.80 $\pm$ 0.52 & 89.60 $\pm$ 0.37 & 80.19 $\pm$ 0.06 & 81.76 \\
GPT-GNN & 59.33 $\pm$ 0.26 & 73.82 $\pm$ 2.06 & 93.01 $\pm$ 0.07 & 94.16 $\pm$ 3.06 & 70.86 $\pm$ 0.34 & 88.60 $\pm$ 0.26 & 81.20 $\pm$ 0.12 & 80.14 \\
% DGI & 75.31 $\pm$ 0.67 & 85.93 $\pm$ 0.37 & 93.49 $\pm$ 0.12 & 96.54 $\pm$ 0.01 & 75.96 $\pm$ 0.05 & 92.94 $\pm$ 0.01 & 83.43 $\pm$ 0.04 \\ 
\midrule
\method & \textbf{76.49 $\pm$ 0.25} & \textbf{85.44 $\pm$ 0.20} & 93.01 $\pm$ 0.05 & 94.49 $\pm$ 0.00 & \textbf{75.82 $\pm$ 0.00} & \textbf{92.74 $\pm$ 0.00} & \textbf{84.24 $\pm$ 0.05} & \textbf{86.32} \\
\bottomrule
\end{tabular}
}
\caption{HIV, Linear, ACC, CV 0.9, last layer}
\end{table}


\begin{table}[!h]
\center
\scalebox{0.72}{
\begin{tabular}{@{}l|ccccccc|c@{}}
\toprule
\multicolumn{1}{l|}{\begin{tabular}[l]{@{}c@{}}SSL methods\end{tabular}} & \multicolumn{1}{c}{bace} & bbbp & clintox & hiv & sider & tox21 & toxcast  & Average\\ \midrule
% Non-Pretrain & \\ 
% \midrule
ContextPred & 73.19 $\pm$ 0.13 & 80.26 $\pm$ 0.14 & 67.41 $\pm$ 0.92 & 75.31 $\pm$ 0.03 & 61.54 $\pm$ 0.29 & 75.52 $\pm$ 0.08 & 66.12 $\pm$ 0.13 & 71.33\\
InfoGraph & 76.88 $\pm$ 0.18 & 85.2 $\pm$ 0.25 & 85.74 $\pm$ 0.46 & 74.5 $\pm$ 0.22 & 60.17 $\pm$ 0.19 & 76.86 $\pm$ 0.11 & 65.51 $\pm$ 0.11 & 74.98\\
GPT-GNN & 65.58 $\pm$ 0.24 & 78.77 $\pm$ 0.12 & 71.83 $\pm$ 0.71 & 70.4 $\pm$ 0.06 & 58.25 $\pm$ 0.24 & 74.15 $\pm$ 0.08 & 63.91 $\pm$ 0.06 & 68.98\\
% DGI & \\ 
\midrule
\method & 79.33 $\pm$ 0.16 & 85.64 $\pm$ 0.35 & 77.98 $\pm$ 0.3 & 76.14$\pm$ 0.11 & 62.71 $\pm$ 0.09 & 79.11 $\pm$ 0.13 & 69.09 $\pm$ 0.07 & 75.71\\
\bottomrule
\end{tabular}
}
\caption{Zinc, Linear, ROC, CV 0.9, last-layer}
\end{table}



\begin{table}[!h]
\center
\scalebox{0.72}{
\begin{tabular}{@{}l|ccccccc|c@{}}
\toprule
\multicolumn{1}{l|}{\begin{tabular}[l]{@{}c@{}}SSL methods\end{tabular}} & \multicolumn{1}{c}{bace} & bbbp & clintox & hiv & sider & tox21 & toxcast  & Average\\ \midrule
% Non-Pretrain & \\ 
% \midrule
ContextPred & 71.43 $\pm$ 0.1 & 79.61 $\pm$ 0.1 & 66.82 $\pm$ 0.78 & 72.37 $\pm$ 0.06 & 60.89 $\pm$ 0.24 & 75.14 $\pm$ 0.13 & 65.61 $\pm$ 0.11 \\
InfoGraph &  \\
GPT-GNN & \\
% DGI & \\ 
\midrule
\method & 79.33 $\pm$ 0.16 & 85.64 $\pm$ 0.35 & 77.98 $\pm$ 0.3 & 76.14$\pm$ 0.11 & 62.71 $\pm$ 0.09 & 79.11 $\pm$ 0.13 & 69.09 $\pm$ 0.07 & 75.71\\
\bottomrule
\end{tabular}
}
\caption{Zinc, Linear, ROC, CV 0.9, penultimate layer}
\end{table}

\begin{table}[]
\center
\scalebox{0.75}{
\begin{tabular}{@{}l|lllllll@{}}
\toprule
\multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Dataset\\ Method\end{tabular}} & \multicolumn{1}{c}{bace} & bbbp & clintox & hiv & sider & tox21 & toxcast \\ \midrule
Non-pretrain &  \\
InfoGraph &  \\
ContextPred & \\
GPT-GNN & \\
DGI & 71.83 $\pm$ 2.32 & 65.85 $\pm$ 1.35 & 81.83 $\pm$ 4.5 & 76.4 $\pm$ 1.56 & 59.57 $\pm$ 0.98 & 75.75 $\pm$ 0.41 & 65.61 $\pm$ 0.27 \\ \midrule
MICRO-Graph &
\end{tabular}
}
\caption{zinc standard agent (scaffold)}
\end{table}


